CMU-Flownet: Exploring Point Cloud Scene Flow Estimation in Occluded Scenario

Occlusions hinder point cloud frame alignment in LiDAR data, a challenge inadequately addressed by scene flow models tested mainly on occlusion-free datasets. Attempts to integrate occlusion handling within networks often suffer accuracy issues due to two main limitations: a) the inadequate use of occlusion information, often merging it with flow estimation without an effective integration strategy, and b) reliance on distance-weighted upsampling that falls short in correcting occlusion-related errors. To address these challenges, we introduce the Correlation Matrix Upsampling Flownet (CMU-Flownet), incorporating an occlusion estimation module within its cost volume layer, alongside an Occlusion-aware Cost Volume (OCV) mechanism. Specifically, we propose an enhanced upsampling approach that expands the sensory field of the sampling process which integrates a Correlation Matrix designed to evaluate point-level similarity. Meanwhile, our model robustly integrates occlusion data within the context of scene flow, deploying this information strategically during the refinement phase of the flow estimation. The efficacy of this approach is demonstrated through subsequent experimental validation. Empirical assessments reveal that CMU-Flownet establishes state-of-the-art performance within the realms of occluded Flyingthings3D and KITTY datasets, surpassing previous methodologies across a majority of evaluated metrics.

==> tool.tex <==
import matplotlib.pyplot as plt

# Data for plotting
models = ['3DFlowNet', 'Noisy-Pseudo', 'Ours(1/8)', 'Ours(1/16)', 'Ours(1/32)', 'Ours(1/64)']
epe = [0.028, 0.068, 0.010, 0.015, 0.026, 0.043]  # End Point Error (EPE)
as_metric = [0.929, 0.628, 0.976, 0.969, 0.942, 0.872]  # Accuracy under threshold (AS)
ar_metric = [0.981, 0.881, 0.991, 0.989, 0.973, 0.942]  # Accuracy Rate (AR)
out_metric = [0.146, 0.438, 0.028, 0.035, 0.074, 0.137]  # Outliers (Out)

# Creating line graphs
plt.figure(figsize=(10, 6))
plt.plot(models, epe, marker='o', label='EPE↓')
plt.plot(models, as_metric, marker='o', label='AS↑')
plt.plot(models, ar_metric, marker='o', label='AR↑')
plt.plot(models, out_metric, marker='o', label='Out↓')

# Adding title and labels
plt.title('Comparison of Scene Flow Estimation Models')
plt.xlabel('Models')
plt.ylabel('Metrics')
plt.xticks(rotation=45)
plt.legend()

# Displaying the plot
plt.tight_layout()
plt.show()

